Learning and Dynamical Models for Sub-seasonal Climate Forecasting: Comparison and Collaboration

Sub-seasonal climate forecasting (SSF) is the prediction of key climate variables such as temperature and precipitation on the 2-week to 2-month time horizon. Skillful SSF would have substantial societal value in areas such as agricultural productivity, hydrology and water resource management, and emergency planning for extreme events such as droughts and wildfires. Despite its societal importance, SSF has stayed a challenging problem compared to both short-term weather forecasting and long-term seasonal forecasting. Recent studies have shown the potential of machine learning (ML) models to advance SSF. In this paper, for the first time, we perform a fine-grained comparison of a suite of modern ML models with start-of-the-art physics-based dynamical models from the Subseasonal Experiment (SubX) project for SSF in the western contiguous United States. Additionally, we explore mechanisms to enhance the ML models by using forecasts from dynamical models. Empirical results illustrate that, on average, ML models outperform dynamical models while the ML models tend to be conservatives in their forecasts compared to the SubX models. Further, we illustrate that ML models make forecasting errors under extreme weather conditions, e.g., cold waves due to the polar vortex, highlighting the need for separate models for extreme events. Finally, we show that suitably incorporating dynamical model forecasts as inputs to ML models can substantially improve the forecasting performance of the ML models. The SSF dataset constructed for the work, dynamical model predictions, and code for the ML models are released along with the paper for the benefit of the broader machine learning community.

==> sections/data.tex <==
\subsection{Ground Truth Dataset Construction}
% ground truth or verification

%To have a fair comparison, we construct the ground truth dataset following the same mechanism in building the verification dataset in the SubX project.

\xlcomment{I think we need to explain why we need the ground truth dataset.}

The ground truth dataset is constructed using the data from NOAA's Climate Prediction Center (CPC) Global Gridded Temperature dataset \cite{xie2010cpc,fan2008global}. The dataset contains data from the Global Telecommunication System (GTS) that is gridded using the Shepard Algorithm~[]. Daily max and min 2m temperature (tmp2m) are available at 0.5 $^\circ$ by 0.5 $^\circ$ spatial resolution from Jan 1, 1979 to present. Moreover, the dataset is commonly applied for verification by NOAA/CPC.

To obtain the ground truth temperature anomalies for week 3 \&4, the preprocessing procedure is conducted as follows: (1) daily 2m temperature at each grid point is computed as the average of daily max and min tmp2m, (2) all the missing values are filled by averaging the daily tmp2m of its spatial/temporal neighbors, (3) the tmp2m at 0.5 $^\circ$ by 0.5 $^\circ$ resolution is linearly interpolated to a grid at 1 $^\circ$ by 1 $^\circ$ with integer latitude and longitude, (4) the daily tmp2m anomalies are computed by subtracting the climatology from the observed daily tmp2m, and (5) the forecasting goal at each date and grid point is the average of the tmp2m anomalies at day 15 to 28, i.e., a two-week period that is 14 days ahead of time. The climatology used in step (4) is a smoothed long-term tmp2m average over 1990 - 2016 for each month-day combination at each grid point. For a given grid point, we first compute the long-term average for each month-day combination, e.g. January 1, from 1990 to 2016, and then temporally smooth the computed long-term average tmp2m at all month-day combinations with a moving average with the window size as 31 days. Since the anomalies are computed by removing climatology, there is no difference if the sequence of subtracting climatology and averaging over each two-week period is alternated.

% Four steps:
% \begin{itemize}
%     \item Fill missing values
%     \item Regrid data
%     \item Compute climatology - average \& smooth the data
%     \item Average two weeks
%     \item Compute anomalies
% \end{itemize}



\subsection{SubX Dataset}
In this work, we consider two SubX models, NASA-GMAO and NCEP-CFSv2. The SubX dataset has two predictive periods, that is a hindcast period and a forecast period. A hindcast period represents the time when a dynamic model re-forecasts the historical events. It can help climate scientists develop and test new models that will improve forecasting. A forecast period has real-time predictions generated from the dynamic models. In this paper, we first evaluate the predictive skills of the SubX models over their forecast periods. In addition, we also explore how to improve ML models' forecasting performance by taking advantage of the high-quality forecasts from the SubX models. 

The hindcast period of the two SubX models is from 1999 to 2015. Due to the data availability, the forecast period considered for the NASA-GMAO model is from July 2017 to June 2020, and the forecast period of the NCEP-CFSv2 model is from July 2017 to Mar 2019. The NASA-GMAO model is initialized every five days while the NCEP-CFSv2 model is initialized in a daily manner. All forecasts include daily values for 45 days beyond the initialization date. The weeks 3 \& 4 outlooks are computed by averaging the forecasts 15 to 28 days beyond each initialization date and subtracting the corresponding climatology computed from the hindcast period.

\xlcomment{I think we should has a subsection here to discuss what dataset ML models use, including targets, covariates and how we pre-process them (move sec VI.A here maybe).}


\subsection{Covariates for Machine Learning models}

For machine learning models, we consider numerous climate variables 
representing the condition of the atmosphere, ocean, and land as covariates. 

% one sentence for each variable why we include it

\noindent\textbf{2m Temperature (tmp2m)} 2m temperature is the air temperature at 2 meters above the surface. Daily tmp2m with the unit degree Celsius over the contiguous U.S. is collected from the dataset that is used for constructing the ground truth dataset.

\noindent\textbf{Soil Moisture (sm)} Monthly soil moisture over the contiguous U.S. from 1948 are collected from NOAA's Climate Prediction Center (CPC) Monthly Soil Moisture dataset \cite{soil_1, soil_2, soil_3} with the unit as mm. 

\noindent\textbf{Sea Surface Temperature (sst)} Daily sea surface temperature is provided by NOAA's Optimum Interpolation Sea Surface Temperature (SST) dataset \cite{reynolds2007daily}. We consider the sst over the Pacific Ocean, delimited by the latitudes 20S to 65N and longitudes 120E to 90W, and North Atlantic Ocean, delimited by the latitudes 20S to 50N and longitudes 20W to 90W.

\noindent\textbf{Geopotential Height (ght), relative humidity (rhum), and sea level pressure (slp)} To capture XXX, geopotential height at 10mb and 500mb over the contiguous U.S. are included in the covariates set. We also obtain the relative humidity near the surface (sigma level 0.995) and sea level pressure (\textit{reasons}). All three climate variables over the contiguous U.S. are provided by the NCEP Reanalysis dataset \cite{reanalysis}. The original temporal resolution of the dataset is 4-times daily. We calculate the daily values by averaging all the data at each date.

\noindent\textbf{Multivariate ENSO Index (MEI)} The bi-monthly Multivariate El Ni\~no/Southern Oscillation (ENSO) index (MEI.v2) is provided from NOAA Physical Sciences Laboratory \cite{zimmerman2016utilizing} []. It is the time series of the leading combined Empirical Orthogonal Function (EOF) of five different variables (sea level pressure, sea surface temperature, zonal and meridional components of the surface wind, and outgoing longwave radiation) over the tropical Pacific basin. % (30°S-30°N and 100°E-70°W)

\noindent\textbf{Madden-Julian Oscillation Index (mjo)} Daily MJO amplitude and phase are obtained from the Australian Government Bureau of Meteorology \cite{MJO}. MJO has dramatic impacts in the mid-latitudes and is a strong contributor to various extreme events in the U.S. The MJO index carries information on the variability in the tropical atmosphere. 

\noindent\textbf{Ni\~no Indexes} To monitor the tropical Pacific, we include weekly ni\~no 1+2, ni\~no 3, ni\~no 34, and ni\~no 4 indexes from NOAA National Weather Service, CPC \cite{reynolds2007daily}. The ni\~no 3.4 index is one of the most commonly used indices to define El Ni\~no and La Ni\~na events. Other indices are used to help characterize the unique nature of each event.  

\noindent\textbf{North Atlantic Oscillation Index (nao)} Daily North Atlantic oscillation index is originally collected by NOAA National Weather Service, CPC \cite{NAO_1, NAO_2}. The daily NAO index is constructed by projecting the daily (00Z) 500mb height anomalies over the Northern Hemisphere onto the loading pattern of the NAO. 

\noindent\textbf{Sudden Stratospheric Warming Index (ssw)} The ssw index we use is the zonal mean winds at 60N at 10hPa computed from the Modern-Era Retrospective Analysis for Research and Applications (MERRA) dataset \cite{gelaro2017modern}. \textit{reason}.

\subsection{Data Preprocessing}
As described in Section \ref{sec: data}, the target variable is tmp2m anomalies for weeks 3 \& 4 over the western U.S., which is also the covariate used for the AutoKNN model. For the other three ML models, we consider two types of climate variables, i.e., spatiotemporal climate variables and temporal climate variables. For spatiotemporal climate variables, we flatten the values at all grid points for each date and compute the top 10 principal components (PCs) for each climate variable separately, base on the PC loadings from 1990 to 2016. The extracted PCs are then normalized by z-scoring on each day of the year. The PC-based features of all spatiotemporal climate variables and the daily temporal variables jointly form the feature set for each date. For XGBoost and Lasso, the covariates used for each forecast are the features of the first available date, i.e., 14 days ahead of the forecasted two-week period. For the Encoder FNN, a historical sequence containing the target date and its temporal neighbors in the past two years is constructed for each date following the same manner described in \cite{heli21}.

==> sections/exp-setup.tex <==
%\subsection{Data Preprocessing}



\xlcomment{I am thinking of moving B and C to section III.}

\subsection{Evaluation Pipeline}
Predictive models are created independently for each month from July 2017 to Jun 2020. The evaluated dates in each month are decided by the forecasting period and temporal resolution of the two SubX models. Each month in the forecasting period is treated as an individual test set. For a given test set, e.g. January 2018, we first construct a set of training-validation pairs using the data from 2000 to 2016. Data from the same month of the year  (e.g., January) in 2012 - 2016 are the five validation sets. Their corresponding training sets consist of the 10 years of data before each validation set. The best hyper-parameters for the month of the year are determined by the average performance over five validations sets. Thus we have twelve sets of the best hyperparameter selected since the relationships between the covariates and target variables vary during a different time at a year. Once the best hyper-parameters are selected, the forecasting model for a given test set is eventually trained using the data over 28 years before the test set. As a result, one model is trained for each month, i.e., each test set, in the forecasting period.
% Do we need to explain why we have one set of hyperparameter for each month?

\subsection{Evaluation Metrics}
In this paper, we consider the following three metrics to evaluate the predictive performance of each forecasting model from different perspectives. Denote $\y^*\in \R^n$ as the vector of ground truth and $\hat{\y}\in \R^n$ as the predicted values. The three evaluation metrics are defined as follows:

\noindent \textbf{Anomaly Correlation Coefficient (ACC)} A measure of the linear association between the forecasts and ground truth that is independent of the mean and variance of the individual distributions. ACC is defined as 
    \begin{equation}
        \text{ACC}=\frac{\text{cov}(\y^*,\hat{\y})}{\sigma_{\y^*}\sigma_{\hat{\y}}}~,
    \end{equation}
    where $\sigma_{\y^*}$ and $\sigma_{\hat{\y}}$ represent the standard deviation of the forecast and ground truth data over the forecasting period, respectively. The $\text{cov}(\y^*,\hat{\y})$ is the covariance between $\y^*$ and $\hat{\y}$. Since the climatology is removed from the data, assuming the forecast $\hat{\y}$ is zero-mean, the metric ACC is equivalent to cosine similarity between $\y^*$ and $\hat{\y}$.
    
\noindent \textbf{Root Mean Square Error (RMSE)} The square root of the average of the squared differences between forecasts and ground truth data. RMSE is defined as 
    \begin{equation}
        \text{RMSE}= \sqrt{\frac{\sum_{i=1}^n(\y^*_i - \hat{\y}_i)^2}{n}}~.
    \end{equation}
    where $\y^*_i$ and $\hat{\y}_i$ are the $i$-th element in $\y$ and $\hat{y}$ respectively.

\noindent \textbf{Relative $R^2$} The relative predictive skill of a given prediction $\hat{\y}$ compared to the best constant predictor $\bar{\y}_{\text{train}}$, i.e., the long-term average of target variable at each date and each target location computed from training set. It is defined as 
\begin{align}
   \text{Relative } R^2 &=1-\text{Relative MSE}\\
   &=
1-\frac{\sum_{i=1}^n(\y^*_i-\hat{\y}_i)^2}{\sum_{i=1}^n(\y^*_i-\bar{\y}_{\text{train}})^2}~, 
\end{align}
where $\bar{\y}_{\text{train}}$ is 0 due to the normalization. A model which achieves a positive relative $R^2$ is, at least, able to predict the sign of $y^*$ accurately. \xlcomment{Do we want to emphasis the sign or do we want to emphasis it is better than climatology?}

All evaluation metrics can be computed in either spatial or temporal manner. If $\y^*$ represents the ground truth tmp2m for a period of time at one location, the metrics evaluate the predictive performance temporally, which is similar to time series forecasting evaluation. If $\y^*$ contains the
ground truth values for all target locations at one date, the metrics are computed in a spatial manner, which evaluates spatially if the forecasts align well with the ground truth data for the given date.


==> sections/table-fig.tex <==
\subsection{Results of SubX models}
\begin{table}[t]
\centering
\caption{Spatial ACC, RMSE, and relative $R^2$ of the two SubX models.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
Method     & 2017         & 2018         & 2019         & 2020         \\ \hline
\multicolumn{5}{|c|}{ACC}                                              \\ \hline
GMAO       & 0.10 (0.09)  & 0.25 (0.05)  & 0.14 (0.05)  & 0.06 (0.07)  \\ \hline
NCEP-CFSv2 & 0.11 (0.05)  & 0.22 (0.03)  & 0.18 (0.06)  & N/A          \\ \hline
\multicolumn{5}{|c|}{RMSE}                                             \\ \hline
GMAO       & 2.83 (0.20)  & 2.42 (0.13)  & 2.84 (0.14)  & 2.44 (0.19)  \\ \hline
NCEP-CFSv2 & 2.12 (0.09)  & 2.45 (0.07)  & 4.14 (0.26)  & N/A          \\ \hline
\multicolumn{5}{|c|}{Relative   R2}                                    \\ \hline
GMAO       & -0.27 (0.12) & -0.31 (0.10) & -1.17 (0.22) & -0.88 (0.20) \\ \hline
NCEP-CFSv2 & -0.34 (0.09) & -0.36 (0.06) & -0.47 (0.13) & N/A          \\ \hline
\end{tabular}}
\label{tab: subx}
\end{table}


\begin{table*}[t]
\centering
\caption{Spatial ACC and relative $R^2$ of NASA-GMAO and ML models.}
\begin{tabular}{|c|c|c|c|c|}
\hline
Method      & Mean         & Median       & 0.25 quantile & 0.75 quantile \\ \hline
\multicolumn{5}{|c|}{ACC}                                                 \\ \hline
GMAO        & 0.16 (0.03)  & 0.19 (0.04)  & -0.17 (0.05)  & 0.49 (0.04)   \\ \hline
AutoKNN     & 0.19 (0.03)  & 0.26 (0.06)  & -0.23 (0.06)  & 0.60 (0.04)   \\ \hline
XGBoost     & 0.13 (0.02)  & 0.13 (0.04)  & -0.12 (0.03)  & 0.41 (0.04)   \\ \hline
Lasso       & 0.11 (0.03)  & 0.13 (0.04)  & -0.16 (0.04)  & 0.44 (0.04)   \\ \hline
Encoder-FNN & 0.12 (0.03)  & 0.13 (0.05)  & -0.16 (0.04)  & 0.48 (0.04)   \\ \hline
\multicolumn{5}{|c|}{Relative   $R^2$}                          \\ \hline
GMAO        & -0.71 (0.10) & -0.24 (0.08) & -1.08 (0.14)  & 0.15 (0.07)   \\ \hline
AutoKNN     & 0.01 (0.01)  & 0.01 (0.02)  & -0.09 (0.01)  & 0.15 (0.02)   \\ \hline
XGBoost     & 0.00 (0.01)  & 0.01 (0.01)  & -0.07 (0.01)  & 0.10 (0.01)   \\ \hline
Lasso       & -0.01 (0.01) & 0.01 (0.01)  & -0.09 (0.01)  & 0.09 (0.01)   \\ \hline
Encoder-FNN & -0.15 (0.04) & 0.01 (0.04)  & -0.34 (0.06)  & 0.23 (0.03)   \\ \hline
\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
\caption{Spatial ACC and relative $R^2$ of NASA-GMAO and ML models for each year.}
\begin{tabular}{|c|c|c|c|c|}
\hline
Method      & 2017         & 2018         & 2019         & 2020                               \\ \hline
\multicolumn{5}{|c|}{ACC}                                                                     \\ \hline
GMAO        & 0.10 (0.09)  & 0.25 (0.05)  & 0.14 (0.05)  & 0.06 (0.07)                        \\ \hline
AutoKNN     & 0.11 (0.08)  & 0.25 (0.04)  & 0.02 (0.05)  & 0.24 (0.06)                        \\ \hline
XGBoost     & 0.18 (0.06)  & 0.18 (0.04)  & 0.03 (0.04)  & 0.09 (0.05)                        \\ \hline
Lasso       & 0.32 (0.06)  & 0.18 (0.04)  & 0.01 (0.05)  & 0.04 (0.07)                        \\ \hline
Encoder-FNN & 0.24 (0.09)  & 0.07 (0.06)  & 0.27 (0.05)  & 0.20 (0.08)                        \\ \hline
\multicolumn{5}{|c|}{Relative   $R^2$}                                               \\ \hline
GMAO        & -0.27 (0.12) & -0.31 (0.10) & -1.17 (0.22) & -0.88 (0.20)                       \\ \hline
AutoKNN     & 0.00 (0.03)  & 0.05 (0.02)  & -0.04 (0.03) & \multicolumn{1}{l|}{0.06   (0.03)} \\ \hline
XGBoost     & 0.03 (0.02)  & 0.05 (0.02)  & -0.06 (0.03) & 0.00 (0.02)                        \\ \hline
Lasso       & 0.04 (0.01)  & 0.01 (0.02)  & -0.03 (0.02) & -0.08 (0.04)                       \\ \hline
Encoder-FNN & -0.27 (0.14) & -0.28 (0.08) & -0.06 (0.06) & 0.03 (0.06)                        \\ \hline
\end{tabular}
\end{table*}



\begin{table*}[t]
\caption{Spatial ACC and relative $R^2$ of NCEP-CFSv2 and ML models.}
\centering

\begin{tabular}{|c|c|c|c|c|}
\hline
Method      & Mean         & Median       & 0.25 quantile & 0.75 quantile \\ \hline
\multicolumn{5}{|c|}{ACC}                                                 \\ \hline
NCEP        & 0.19 (0.02)  & 0.30 (0.03)  & -0.20 (0.04)  & 0.59 (0.02)   \\ \hline
AutoKNN     & 0.12 (0.02)  & 0.14 (0.03)  & -0.17 (0.04)  & 0.49 (0.02)   \\ \hline
XGBoost     & 0.19 (0.02)  & 0.24 (0.02)  & -0.09 (0.03)  & 0.49 (0.02)   \\ \hline
Lasso       & 0.12 (0.02)  & 0.14 (0.03)  & -0.17 (0.03)  & 0.45 (0.02)   \\ \hline
Encoder-FNN & 0.19 (0.02)  & 0.30 (0.05)  & -0.31 (0.04)  & 0.67 (0.02)   \\ \hline
\multicolumn{5}{|c|}{Relative   $R^2$}                     \\ \hline
GMAO        & -0.37 (0.05) & -0.05 (0.04) & -0.76 (0.08)  & 0.29 (0.03)   \\ \hline
AutoKNN     & 0.02 (0.01)  & 0.02 (0.01)  & -0.09 (0.01)  & 0.16 (0.01)   \\ \hline
XGBoost     & 0.04 (0.01)  & 0.05 (0.01)  & -0.06 (0.01)  & 0.14 (0.01)   \\ \hline
Lasso       & 0.01 (0.01)  & 0.01 (0.01)  & -0.07 (0.01)  & 0.12 (0.01)   \\ \hline
Encoder-FNN & -0.21 (0.03) & 0.01 (0.03)  & -0.51 (0.06)  & 0.30 (0.02)   \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{Spatial ACC and relative $R^2$ of NCEP-CFSv2 and ML models for each year.}
\centering

\begin{tabular}{|c|c|c|c|}
\hline
Method      & 2017         & 2018         & 2019                                \\ \hline
\multicolumn{4}{|c|}{ACC}                                                       \\ \hline
NCEP        & 0.11 (0.05)  & 0.22 (0.03)  & 0.18 (0.06)                         \\ \hline
AutoKNN     & 0.18 (0.05)  & 0.17 (0.02)  & \multicolumn{1}{l|}{-0.23 (0.05)}   \\ \hline
XGBoost     & 0.13 (0.04)  & 0.27 (0.02)  & -0.08 (0.03)                        \\ \hline
Lasso       & 0.12 (0.03)  & 0.18 (0.02)  & -0.15 (0.06)                        \\ \hline
Encoder-FNN & 0.20 (0.05)  & 0.12 (0.03)  & 0.53 (0.05)                         \\ \hline
\multicolumn{4}{|c|}{Relative   $R^2$}                                \\ \hline
NCEP        & -0.34 (0.09) & -0.36 (0.06) & -0.47 (0.13)                        \\ \hline
AutoKNN     & 0.02 (0.03)  & 0.05 (0.01)  & \multicolumn{1}{l|}{-0.14   (0.03)} \\ \hline
XGBoost     & 0.02 (0.01)  & 0.06 (0.01)  & -0.02 (0.01)                        \\ \hline
Lasso       & 0.00 (0.01)  & 0.01 (0.01)  & -0.03 (0.02)                        \\ \hline
Encoder-FNN & -0.21 (0.07) & -0.23 (0.04) & -0.12 (0.12)                        \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{The spatial results of ML models with and without NASA-GMAO forecasts.}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method  & Mean          & Median        & 0.25 quantile  & 0.75 quantile \\ \hline
GMAO    & 0.16 (0.03)   & 0.19 (0.04)   & -0.17 (0.05)   & 0.49 (0.04)   \\ \hline
XGBoost & 0.13 (0.02)   & 0.13 (0.04)   & -0.12 (0.03)   & 0.41 (0.04)   \\ \hline
Lasso   & 0.11   (0.03) & 0.13   (0.04) & -0.16   (0.04) & 0.44   (0.04) \\ \hline
\multicolumn{5}{|c|}{Without   GMAO   Forecasts}                         \\ \hline
XGBoost & 0.09   (0.02) & 0.12   (0.03) & -0.17   (0.04) & 0.34   (0.03) \\ \hline
Lasso   & 0.12   (0.03) & 0.16   (0.04) & -0.11   (0.04) & 0.43   (0.03) \\ \hline
\multicolumn{5}{|c|}{With   GMAO Forecasts}                              \\ \hline
XGBoost & 0.13   (0.02) & 0.14   (0.04) & -0.14   (0.04) & 0.40   (0.03) \\ \hline
Lasso   & 0.16   (0.03) & 0.18   (0.04) & -0.10   (0.05) & 0.49   (0.03) \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{The spatial results of ML models with and without NCEP-CFSv2 forecasts.}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method  & Mean          & Median        & 0.25 quantile  & 0.75 quantile \\ \hline
NCEP    & 0.19 (0.02)   & 0.30 (0.03)   & -0.20 (0.04)   & 0.59 (0.02)   \\ \hline
XGBoost & 0.19 (0.02)   & 0.24 (0.02)   & -0.09 (0.03)   & 0.49 (0.02)   \\ \hline
Lasso   & 0.12 (0.02)   & 0.14 (0.03)   & -0.17 (0.03)   & 0.45 (0.02)   \\ \hline
\multicolumn{5}{|c|}{Without   NCEP Forecasts}                           \\ \hline
XGBoost & 0.15   (0.02) & 0.21   (0.03) & -0.16   (0.03) & 0.46   (0.02) \\ \hline
Lasso   & 0.19   (0.01) & 0.21   (0.02) & 0.02   (0.02)  & 0.44   (0.02) \\ \hline
\multicolumn{5}{|c|}{With   NCEP Forecasts}                              \\ \hline
XGBoost & 0.18   (0.02) & 0.23   (0.02) & -0.11   (0.03) & 0.46   (0.02) \\ \hline
Lasso   & 0.23   (0.02) & 0.25   (0.02) & 0.00   (0.03)  & 0.53 (0.02)   \\ \hline
\end{tabular}
\end{table*}
We consider both spatial and temporal forecasting performance for SubX and ML models.
\subsection{Analysis and Exploration}
\subsubsection{Combination of ML models and SubX forecasts}
In this section we explore how the forecasting performance is when ML models take the advantage of SubX forecasts.
\subsubsection{When do forecasting models fail?}
The experiment
\subsubsection{Hindcast}


\begin{figure}[ht]
    \centering
    \subfigure[ACC]{\includegraphics[width=0.4\textwidth]{images/gmao-acc.png}}

    \subfigure[Relative \text{$R^2$}]{\includegraphics[width=0.4\textwidth]{images/gmao-r2.png}}
    %\vspace{-2mm}
    \caption{The temporal results of NASA-GMAO and ML models.}
     \label{fig:gmao}
\end{figure}

\begin{figure}[ht]
    \centering
    \subfigure[ACC]{\includegraphics[width=0.4\textwidth]{images/ncep-acc.png}}

    \subfigure[Relative \text{$R^2$}]{\includegraphics[width=0.4\textwidth]{images/ncep-r2.png}}
    %\vspace{-2mm}
    \caption{The temporal results of NCEP-CFSv2 and ML models.}
     \label{fig:ncep}
\end{figure}


\begin{figure}[ht]
    \centering
    \subfigure[ACC]{\includegraphics[width=0.4\textwidth]{images/ncep-acc-wo2019.png}}

    \subfigure[Relative \text{$R^2$}]{\includegraphics[width=0.4\textwidth]{images/ncep-r2-wo2019.png}}
    %\vspace{-2mm}
    \caption{The temporal results of NCEP-CFSv2 and ML models without considering the first three months in 2019.}
     \label{fig:ncep_wo_2019}
\end{figure}


\begin{figure}[ht]
    \centering
    \subfigure[NASA-GMAO]{\includegraphics[width=0.4\textwidth]{images/gmao-feature.png}}

    \subfigure[NCEP-CFSv2]{\includegraphics[width=0.4\textwidth]{images/ncep-feature.png}}
    \caption{The influence of different feature sets.}
     \label{fig:feature}
\end{figure}


\begin{figure}[ht]
    \centering
    \subfigure[NASA-GMAO]{\includegraphics[width=0.4\textwidth]{images/gmao-hist.png}}

    \subfigure[NCEP-CFSv2]{\includegraphics[width=0.4\textwidth]{images/ncep-hist.png}}
    \caption{The temporal results of SubX models and ML models.}
     \label{fig:temp}
\end{figure}


\begin{figure}[ht]
    \centering
    \subfigure[ACC]{\includegraphics[width=0.4\textwidth]{images/ml-gmao-acc.png}}

    \subfigure[Relative \text{$R^2$}]{\includegraphics[width=0.4\textwidth]{images/ml-gmao-r2.png}}
    \caption{The temporal results of ML models with and without NASA-GMAO forecasts.}
     \label{fig:ml-gmao}
\end{figure}



\begin{figure}[ht]
    \centering
    \subfigure[ACC]{\includegraphics[width=0.4\textwidth]{images/ml-ncep-acc.png}}

    \subfigure[Relative \text{$R^2$}]{\includegraphics[width=0.4\textwidth]{images/ml-ncep-r2.png}}
    \caption{The temporal results of ML models with and without NCEP-CFSv2 forecasts.}
     \label{fig:ml-ncep}
\end{figure}



\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{images/ml-ncep-acc-wo2019.png}
    \caption{The temporal results of ML models with and without NCEP-CFSv2 forecasts without considering 2019.}
     \label{fig:ml-ncep-wo2019}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{images/var.png}
    \caption{The spatial variance over time for western US.}
     \label{fig:var}
\end{figure}
